Chiral Effective Theory Methods and their Application to the Structure of Hadrons from Lattice QCD

For many years chiral effective theory (ChEFT) has enabled and supported lattice QCD calculations of hadron observables by allowing systematic effects from unphysical lattice parameters to be controlled. In the modern era of precision lattice simulations approaching the physical point, ChEFT techniques remain valuable tools. In this review we discuss the modern uses of ChEFT applied to lattice studies of hadron structure in the context of recent determinations of important and topical quantities. We consider muon g-2, strangeness in the nucleon, the proton radius, nucleon polarizabilities, and sigma terms relevant to the prediction of dark-matter-hadron interaction cross-sections, among others.

==> Figures/g-2_compare.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8502.00,4534.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(511,-4050){\makebox(0,0){\strut{}$500$}}%
      \put(965,-4050){\makebox(0,0){\strut{}$550$}}%
      \put(1418,-4050){\makebox(0,0){\strut{}$600$}}%
      \put(1871,-4050){\makebox(0,0){\strut{}$650$}}%
      \put(2324,-4050){\makebox(0,0){\strut{}$700$}}%
      \put(2777,-4050){\makebox(0,0){\strut{}$750$}}%
      \csname LTb\endcsname%
      \put(3140,-262){\makebox(0,0)[l]{\strut{}Dispersion rel.~~\textcolor{red}{[PDG, 2014]}~~\cite{PDG2014}}}%
      \put(3140,-658){\makebox(0,0)[l]{\strut{}$u,d,s_Q,c_Q$~~Wilson~~\textcolor{red}{[Mainz, this work]}~~$N_f=2$}}%
      \put(3140,-856){\makebox(0,0)[l]{\strut{}$u,d,s,c$~~TM~~\textcolor{red}{[ETMC, 2013]}~~\cite{Burger:2013jya}~~$N_f=2+1+1$}}%
      \put(3140,-1451){\makebox(0,0)[l]{\strut{}$u,d,s_Q$~~Wilson~~\textcolor{red}{[Mainz, this work]}~~$N_f=2$}}%
      \put(3140,-1649){\makebox(0,0)[l]{\strut{}$u,d,s_Q$~~Wilson~~\textcolor{red}{[Mainz, 2011]}~~\cite{DellaMorte:2011aa}~~$N_f=2$}}%
      \put(3140,-1847){\makebox(0,0)[l]{\strut{}$u,d,s$~~TM~~\textcolor{red}{[ETMC, 2013]}~~\cite{Burger:2013jya}~~$N_f=2+1+1$}}%
      \put(3140,-2045){\makebox(0,0)[l]{\strut{}$u,d,s$~~DWF~~\textcolor{red}{[RBC-UKQCD, 2012]}~~\cite{Boyle:2011hu}~~$N_f=2+1$}}%
      \put(3140,-2243){\makebox(0,0)[l]{\strut{}$u,d,s$\, Asqtad (lin.)~~\textcolor{red}{[Aubin et al., 2007]}~~\cite{Aubin:2012me}~~$N_f=2+1$}}%
      \put(3140,-2441){\makebox(0,0)[l]{\strut{}$u,d,s$\, Asqtad (quad.)~~\textcolor{red}{[Aubin et al., 2007]}~~\cite{Aubin:2012me}~~$N_f=2+1$}}%
      \put(3140,-2837){\makebox(0,0)[l]{\strut{}$u,d$~~Wilson~~\textcolor{red}{[Mainz, this work]}~~$N_f=2$}}%
      \put(3140,-3036){\makebox(0,0)[l]{\strut{}$u,d$~~Wilson~~\textcolor{red}{[Mainz, 2011]}~~\cite{DellaMorte:2011aa}~~$N_f=2$}}%
      \put(3140,-3234){\makebox(0,0)[l]{\strut{}$u,d$~~TM~~\textcolor{red}{[ETMC, 2013]}~~\cite{Burger:2013jya}~~$N_f=2+1+1$}}%
      \put(3140,-3432){\makebox(0,0)[l]{\strut{}$u,d$~~TM~~\textcolor{red}{[ETMC, 2011]}~~\cite{Feng:2011zk}~~$N_f=2$}}%
      \put(511,-559){\makebox(0,0)[l]{\strut{}\textsc{Preliminary}}}%
      \put(3140,-1054){\makebox(0,0)[l]{\strut{}$u,d,s,c$~~}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1667,-4380){\makebox(0,0){\strut{}$a_\mu^{\mathrm{HLO}} \times 10^{10}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{g-2_compare}}%
    \gplfronttext
  \end{picture}%
\endgroup

